Emerging Convolutions for Generative Normalizing Flows

Generative flows are attractive because they admit exact likelihood optimization and efficient image synthesis. Recently, Kingma & Dhariwal (2018) demonstrated with Glow that generative flows are capable of generating high quality images. We generalize the 1 x 1 convolutions proposed in Glow to invertible d x d convolutions, which are more flexible since they operate on both channel and spatial axes. We propose two methods to produce invertible convolutions that have receptive fields identical to standard convolutions: Emerging convolutions are obtained by chaining specific autoregressive convolutions, and periodic convolutions are decoupled in the frequency domain. Our experiments show that the flexibility of d x d convolutions significantly improves the performance of generative flow models on galaxy images, CIFAR10 and ImageNet.

==> sections/details.tex <==
%!TEX root = ../main.tex


Models are optimized with settings identical to \cite{kingma2018glow}. The optimizer Adamax is used with a learning rate of 0.001. Coupling layers contain neural networks with three convolution layers. The first and last convolution are $3 \times 3$ and the center convolution is $1 \times 1$. The two hidden layers have $W$ (width) channels and ReLU activations. A flow module consists of an actnorm layer, a mixing layer and a coupling layer. A mixing layer is either a $1 \times 1$ convolution (Glow) or a $3 \times 3$ (emerging or periodic) convolution. A forward pass of the entire model uses $D$ flows per level $L$. At the end of a level the squeeze operation reduces the spatial dimensions by two, and increases the channel dimensions by four. 




\begin{table}[H]
\centering
\caption{Experimental setup on galaxy image modeling.}
\begin{tabularx}{.47\textwidth}{l X X X l }
\hline
Model & $L$ & $D$ & $W$ & batchsize \\ \hline 
$1 \times 1$ & 3 & 8 & 512 & 256 \\
Periodic $3 \times 3$ & 3 & 8 & 510 & 256 \\
Emerging $3 \times 3$ & 3 & 8 & 510 & 256 \\ \hline 
\end{tabularx}
\end{table}

In the MAF model, $1 \times 1$ convolutions are succeeded (not replaced) by two MAF layers with opposite autoregressive order. MAF layers have the same structure as coupling layers, with the difference that the two hidden layers have 96 channels.  

\begin{table}[H]
\centering
\caption{Experimental setup on CIFAR10}
\begin{tabularx}{0.47\textwidth}{l X X X l }
\hline
Model & $L$ & $D$ & $W$ & batchsize \\ \hline 
Glow & 3 & 32 & 512 & 256 \\
MAF & 3 & 32 & 462 & 256 \\
Emerging & 3 & 32 & 512 & 256 \\ \hline 
\end{tabularx}
\end{table}

The models constrained in size are tested on CIFAR10 and have a different number of flows ($D$) per level. The other hyperparameters remain unchanged.

\begin{table}[H]
\centering
\caption{Experimental setup with constrained model size}
\begin{tabularx}{0.47\textwidth}{l X X l }
\hline
Model & $L$ & $W$ & batchsize \\ \hline 
Glow & 3 & 512 & 256 \\
Emerging & 3 & 507 & 256 \\ \hline 
\end{tabularx}
\end{table}



\begin{table}[H]
\centering
\caption{Experimental setup on ImageNet}
\begin{tabularx}{0.47\textwidth}{l l X X X l }
\hline
Experiment & Dataset & $L$ & $D$ & $W$ & batchsize \\ \hline 
Glow & ImageNet 32 & 3 & 48 & 512 & 256 \\
Emerging & ImageNet 32 & 3 & 48 & 512 & 256 \\ \hline 
Glow & ImageNet 64 & 3 & 48 & 512 & 128 \\
Emerging & ImageNet 64 & 3 & 48 & 512 & 128 \\ \hline 
\end{tabularx}
\end{table}


The experiments that compare parameterizations of the $1 \times 1$ convolutions all use the same hyperparameters, $L=3$, $D=8$, $W=512$, and $\text{batchsize}=256$.

